Privacy Preserving and Resilient RPKI

Resource Public Key Infrastructure (RPKI) is vital to the security of inter-domain routing. However, RPKI enables Regional Internet Registries (RIRs) to unilaterally takedown IP prefixes - indeed, such attacks have been launched by nation-state adversaries. The threat of IP prefix takedowns is one of the factors hindering RPKI adoption. In this work, we propose the first distributed RPKI system, based on threshold signatures, that requires the coordination of a number of RIRs to make changes to RPKI objects; hence, preventing unilateral prefix takedown. We perform extensive evaluations using our implementation demonstrating the practicality of our solution. Furthermore, we show that our system is scalable and remains efficient even when RPKI is widely deployed.

==> system.tex <==
\section{System details}

\subsection{System and Threat Model}

\label{sec:system-threat-model}

\kris[inline]{
	What are the assumptions we make?\\
	Which adversaries do we consider and which not?
}

In this section, first, we state the threat model of existing RPKI before introducing the threat model in our system. We introduce different threat models from MPC literature, along with the motivation behind each of them, that our solution supports. Then, we introduce the system and communication model we use in our work.

%We will be using standard terminology from the MPC literature.


\subsubsection{RPKI threat model}
\kris[inline]{Existing threat model of RPKI\\
	Why is this threat model not sufficient?}

RPKI uses centralized authorities, similar to traditional PKI, who are trusted.
That is, the possibility of the centralized authorities acting maliciously and the compromise of the RPKI are not part of the threat model.
A malicious RIR can revoke and/or delete certificates and ROAs issues from its repository.
Such a system creates an imbalance of power that is unlike the distributed nature of BGP.
The power imbalance with RPKI is greater than Web PKI as only the RIRs can issue certificates to its children in RPKI while in a Web PKI the child has the possibility to request certificates from other CAs.
Furthermore, court orders are not considered threats and hence, it opens up the possibility for nation states to perform coarse-grained censorship.
In fact, RIRs act upon orders from law enforcement.
\kris[inline]{Add reference to Dutch LEA to RIPE and other reference to RIR-LEA pages.}


\subsubsection{Our threat Model}
\label{sec:threat-model}

In our distributed RPKI system, we consider a stronger threat model than the existing RPKI system.
In addition to the threats considered in the existing system, we do not consider the RIRs to be entirely trustworthy.
To be more accurate, we distribute trust so that individual RIRs do not need to be completely trusted.
\kris[inline]{Outline the treat model in simple terms before introducing MPC terminology...link the two}
% What do we mean by trust here?
% It might be better to state it in simple words
% Trust in what and what not?

We consider the guarantees that our distributed RPKI system provides.
We introduce standard MPC terminology to describe threat models in a distributed setting.
We consider adversary power, that is, whether an adversary is passive or active.
Then, we describe the guarantees that can be achieved when the threshold of honest parties varies.
Finally, we describe which guarantees our solution supports and how it translates to the threats against RPKI.


\paragraph{Honest-but-curious vs.~malicious security.}

MPC protocols can be classified in terms of the power of the adversary.
An adversary can be \emph{honest-but-curious} or \emph{malicious}.
An honest-but-curious adversary follows the protocol while a malicious adversary does not follow the protocol and might actively disrupt the protocol.
Security against honest-but-curious adversary is sufficient in many real life scenarios.
If the RIRs trust each other not to act maliciously and instead consider each other to be a necessary check on each other's operation, a protocol secure against honest-but-curious adversary is sufficient.
Such a protocol keeps the signing key away from any internal adversaries and curious employees at the RIRs.
On the one hand, a malicious adversary has full control over the RIRs and can disrupt the protocol.
For instance, it can send wrong values or delay the sending of values.
On the other hand, honest-but-curious adversaries are assumed to provide the correct inputs during the protocol so that no checks on the correctness of the inputs needs to performed.
As might be obvious, a protocol against malicious adversaries provides stronger security guarantees.
However, stronger security comes at the cost of efficiency.
Not only is it harder but it is also less efficient to achieve security against malicious adversaries than against honest-but-curious adversaries.
The difference in the efficiency depends on the specific protocol.

\paragraph{Honest vs.~dishonest majority.}

Let $n$ be the number of RIRs participating in the distributed RPKI system.
During the execution of a threshold signature protocol, a threshold $ t $ number of RIRs need to be available for the protocol to be successfully executed.
When a majority of the RIRs are honest, a threshold $ t \leq \lfloor (n-1)/2 \rfloor $ of parties are needed to sign, then it is called \emph{honest majority}.
When a minority of the RIRs are honest, that is, $ t < n $, the protocol is said to be secure for a \emph{dishonest majority}.
Honest majority protocols are usually faster than dishonest majority protocols and are more beneficial when the availability of the distributed RPKI is of utmost importance.
Honest majority protocols can be used even if some of the RIRs lose their key share as long as at least three-out-of-five RIRs are available and have their key share.
However, there are situations where a dishonest majority protocol might be needed as it provides stronger security such that the adversary needs to corrupt all the parties to be able to access the signing key.
A dishonest majority protocol might also be required when the signature should only be created when there is unanimity among the RIRs.
However, dishonest majority protocols are vulnerable to unavailability when any one of the RIRs are unavailable or crash. 
Hence, these two models provide an availability-security trade-off.

\kris[inline]{Add reference to backup the claim that the RIRs do not collude is a reasonable assumption}

\kris[inline]{Add reference to the recent case of ARIN being fooled into allocating IP space to malicious groups. Explain how this could be prevented by RPKI. Then, state that an honest party would not have had the possibility to go to the court in certain cases.}

\kris[inline]{Explain why transparency + Consent is insufficient. Prevention is better than cure. The possibility to take back address blocks from scammers is useful}
% https://krebsonsecurity.com/2019/05/a-tough-week-for-ip-address-scammers/
% https://www.spamhaus.org/news/article/778/network-hijacking-the-low-down



\subsubsection{System and Communication Model}
\label{sec:system-model}

Our system incorporates all parts of the RPKI that requires generating signatures, which includes the creation of signed objects, ROAs, as well as signing of the resource certificates of children and the issuance of CRLs.
Unlike traditional RPKI, we propose a distributed RPKI system using MPC such that a ROA cannot be signed by a single RIRs on its own.
There are five RIRs and hence, our system includes all of them in the signing process.
Thus, we use $ n = 5 $ in our system.
\kris[inline]{Only meaningful if threshold crypto has already been introduced}


Our system focuses on the role of RIRs as CAs in RPKI.
In this regard, we focus on the key generation and the signing operation in a distributed RPKI system, such that no RIR has access to the signing key.
RIRs create their shares of the secret key.
They have access only to these shares and not to the secret key.
Thus, RIRs cannot unilaterally sign ROAs of ASes or revoke the associated end-entity certificate.

We inherit the communication model from the underlying MPC protocols.
More specifically, we assume the existence of a synchronous communication network where the protocol is executed in rounds~\cite{DBLP:conf/focs/Canetti01,DBLP:conf/tcc/KatzMTZ13}.
The communication between the RIRs is implemented and run on a point-to-point network.
Furthermore, we assume that the RIRs securely communicate with each other using a TLS connection with authenticated endpoints.

\subsection{System setup}

\kris[inline]{
	System overview\\
	How is this system wrt. to existing RPKI ecosystem?\\
	What needs to be changed and what not?\\
	What are the components of the system?\\
	Is it easy to deploy? Why?\\
	Are there assumptions that you make in this system?\\
	Is it fully automated?\\
	Security evaluation\\
	If not, why? Which part requires human intervention?\\
	Diagram?
}


% Not fully automatic. As the RIRs need to check whether or not they agree with the ROAs change, we will argue that our solution is not fully automated. Furthermore, complete automation is not desired as we want to have checks in place.
\subsection{MPC protocol phases}

\kris[inline]{High level description}

\subsubsection{Key generation}

\subsubsection{ROA signing}


\subsection{Security analysis}


\subsection{Deployment scenarios}

\kris[inline]{Case studies: 1. where RIRs disagree (RIPE and ARIN in the FBI case 2011), 2. where there is a legitimate reason to revoke an IP-address block from an INR holder (ARIN case)}

%1. For the same legal notice, RIRs behave differently

%https://www.internetgovernance.org/2011/11/23/in-important-case-ripe-ncc-seeks-legal-clarity-on-how-it-responds-to-foreign-court-orders/
%http://images.spaceref.com/news/2011/ProtectiveOrder.pdf
%
%https://www.ripe.net/publications/news/about-ripe-ncc-and-ripe/ripe-ncc-to-seek-clarification-from-dutch-court-on-police-order-to-temporarily-lock-registration
%https://www.ripe.net/publications/news/about-ripe-ncc-and-ripe/ripe-nccs-case-against-the-state-of-the-netherlands-dismissed
%https://www.ripe.net/publications/news/about-ripe-ncc-and-ripe/summons-of-the-ripe-ncc-against-the-state-of-the-netherlands

- WAN: 5 RIRs in five continents
- LAN: Each RIR with a server in all the other regions






